Zero-Shot Dense Retrieval with Momentum Adversarial Domain Invariant Representations

Dense retrieval (DR) methods conduct text retrieval by first encoding texts in the embedding space and then matching them by nearest neighbor search. This requires strong locality properties from the representation space, i.e, the close allocations of each small group of relevant texts, which are hard to generalize to domains without sufficient training data. In this paper, we aim to improve the generalization ability of DR models from source training domains with rich supervision signals to target domains without any relevant labels, in the zero-shot setting. To achieve that, we propose Momentum adversarial Domain Invariant Representation learning (MoDIR), which introduces a momentum method in the DR training process to train a domain classifier distinguishing source versus target, and then adversarially updates the DR encoder to learn domain invariant representations. Our experiments show that MoDIR robustly outperforms its baselines on 10+ ranking datasets from the BEIR benchmark in the zero-shot setup, with more than 10% relative gains on datasets with enough sensitivity for DR models' evaluation. Source code of this paper will be released.

==> backup/1-intro.tex <==
\section{Introduction}
\label{sec:intro}

% \red{[Dense retrieval is exciting]}
Retrieving relevant information is an important first step of the pipeline for many natural language processing (NLP) and information retrieval (IR) tasks, such as open question answering~\citep{chen-etal-2017-reading} and passage ranking~\citep{monobert}.
Different from conventional sparse retrieval methods such as BM25~\citep{bm25}, dense retrieval (DR) \citep{ict,dpr,ance} encodes queries and documents into a dense embedding space and retrieves relevant documents for a query by searching for its nearest neighbors in the embedding space.
It has been shown to outperform its sparse counterparts in a variety of tasks, in terms of both effectiveness and efficiency.


% \red{[Dense retrieval underperforms on out-of-domain data]}
\cx{more insights on why DR is hard to generalize to unseen data. 1) in comparison to BOW model where there is exact match as lower bound, but zero DR can be random 2) in comparison to classification problems, which needs a boundary while DR is KNN; .}
Despite its exciting power, DR's training typically requires a large amount of in-domain labeled data.
More often than not, annotation is expensive and hard to obtain, especially for special domains such as biomedical search.
If we bypass the labeling difficulty and directly apply a trained DR model to another new domain, it typically fails to generalize well and significantly underperforms baselines such as BM25~\citep{beir}.
In this paper, we aim to tackle this zero-shot transfer challenge for DR, under the setting that no relevance label is available for the target domain.
% \red{[evidence from embedding space analyses?]}



% \red{[A key challenge is how to perform domain adaptation for dense retrieval; more difficult than classifiation]}
\cx{continue discussion \#2 in previous paragraph here. show why classification is a boundary and DR is KNN and needs locality for every potential query---while the query can be allocated anywhere in the space. Then leads to the difficulty it brings to our existing UDA methods, as it increases the variance in the adversarial training (every samples might be very different from others so we need momentum.)}
\cx{I agree that we need a Figure 1 here to help motivate using momentum in ADDA.}
Previously, domain adaptation has been studied intensively for classification tasks~\citep{dann,adda}.
However, dense retrieval is intrinsically different from classification:\ for classification, the model only needs to learn decision boundaries of classes, while for DR, the model needs to learn a distance metric for the entire embedding space that reflects relevance between queries and passages.
On the other hand, in the embedding space for a classification task, data points are often separated into several clusters, while in DR's embedding space they are more uniformly distributed (see Figure 3 of the paper by \citet{dann} and \Cref{fig:tsne} of this paper).
These factors make domain adaptation for DR more challenging and necessitate new methods.


\input{fig-rerank}


% \red{[our methods]}
\cx{I prefer to start with the Momentum part, as that is our main novelty and then describe the adversarial part and DIR part, to complete the picture.}
In this paper, we propose a novel method, \textbf{Mo}mentum Adversarial \textbf{D}omain \textbf{I}nvariant \textbf{R}epresentation (\model), to improve DR models' zero-shot generalization ability to new domains.
% In addition to the encoder model of dense retrieval,
We introduce an auxiliary domain classifier that is trained to discriminate source domain embeddings from the target domain ones.
The DR model's encoder itself, on the other hand, is not only updated to encode queries and relevant documents together, but also adversarially trained to confuse the domain classifier by pushing both domains towards each other in the embedding space.
Since the data points of the two domains do not have nice structures as in classification tasks, na\"ively applying existing methods works poorly.
% In order to improve training stability,
We instead use the \textit{momentum} method:\ before the DR encoder performs an adversarial step, the domain classifier is updated multiple times, each time with a batch that is saved from previous iterations.
The method improves the quality and robustness of the adversarial training process.

% \red{[summary of experiments]}
We conduct experiments to show the effectiveness of \model{} on 15 datasets from the BEIR benchmark~\citep{beir}.
We choose ANCE~\citep{ance} as the backbone DR model and train the model on the source domain dataset MS MARCO~\citep{msmarco}, although \model{} can also be easily applied to other DR models and datasets.
Empirically, \model{} provides robust improvement compared to the baseline ANCE model without any relevance labels from the target domain datasets.

% \red{[contributions]}
\cx{I often don't explitily write down the list of contributions. I prefer to make the first two very clear, one each in previous two paragraphs. and then we use the last paragraph to deliver our deep insight, that we are able to push queries from target to their similar source queries and help convey the learned relevance for ZeroDR. }
Our contributions are as follows.
First, we propose a novel method to learn domain invariant representations to improve DR models' performance on target domains.
Second, we conduct extensive experiments to show the effectiveness of \model{} in the zero-shot transfer setting on the BEIR benchmark.
Third, we provide analyses to show that our method indeed makes the representation space more domain invariant, and this further leads to better ranking performance.




==> backup/2-method.tex <==
\section{Training Domain Invariant Representations for Dense Retrieval}

In this section, we describe the modeling details of \model{}.
The \model{} model consists of two parts:\ the DR encoder $g$ and a domain classifier $f$.
\model's training concerns three loss functions:\ a \textit{ranking} loss, a \textit{discrimination} loss, and an \textit{adversarial} loss.
The ranking loss trains the encoder to pull relevant documents towards the query while pushing away irrelevant ones, the discrimination loss pushes the domain classifier to distinguish embeddings from the two domains, and the adversarial loss pushes the encoder to generate domain invariant representations.

\model{} is trained in the zero-shot dense retrieval setting (ZeroDR).
In many search scenarios outside web search, it is easy to obtain unlabeled queries and documents, but annotating the relevance between them requires expensive manual effort and sometimes even strong domain expertise.
Therefore, in ZeroDR, we have access to queries and documents from both source and target domains, but relevance labels are available only in the source domain.


\subsection{Training the Encoder with Ranking Loss}

We adopt the dual encoder design that has been widely used in DR.
The DR encoder $g$ takes as input a piece of text (query or document) and encodes it into a dense vector.
For a query--document pair $x=(q, d)$, we compute their relevance score as
\begin{equation}
    r(x)=\mathrm{sim}(g(q;\theta_g),g(d;\theta_g)),
\end{equation}
where $\mathrm{sim}$ is a vector similarity function and $\theta_g$ is the collection of parameters of $g$.

At each iteration, we sample from the source domain query--document pairs and their relevance labels.
Each pair is $x^s=(q^s,d^s)$ and its label is $y^s$.
When $y^s=1$, i.e., $q^s$ and $d^s$ are relevant, we further denote the positive query--document pair as $x^{s+}$;
similarly, when $y^s=0$, denote the nagative pair as $x^{s-}$.
The encoder $g$ encodes these pairs and is then updated by minimizing the \textit{ranking loss} $L_R$:
% \cx{write down the full details of this loss, e.g., with ANCE negatives.}
\begin{equation}
    \min_{\theta_g} \sum_{x^{s+}} \sum_{x^{s-}}
    L_R(r(x^{s+}), r(x^{s-})). \label{eqn:loss-ranking}
\end{equation}
In this paper, we follow the settings of ANCE~\citep{ance}:\ $L_R$ is the negative log likelihood (NLL) loss,
% \cx{write down NLL loss in your notation.},
$g$ has the same architecture as RoBERTa-base~\citep{roberta} and outputs the embedding of the last layer's \textsc{[CLS]} token, and $y^s$ is constructed from using the being-optimized DR model to retrieve global hard negatives.
It is worth noting that we choose ANCE simply because it is the state of the art, but \model{} can also build upon other DR models.

\subsection{Training the Domain Classifier with Discrimination Loss and Momentum Queue}
\label{sec:discrimination}

% \cx{You need to first recap your motivation of ZeroDR here and also formally definite your setting (UDA setup). Use a new 1st paragraph here.}

The domain classifier $f$ predicts the probability of whether an input embedding is from the source domain.
We choose a single-layer feed-forward network for $f$, which has been shown in preliminary experiments to have sufficient expressiveness in the high-dimensional embedding space:
\begin{equation}
    f(\mathbf{e}) = \mathrm{softmax}(W_f\mathbf{e}),
\end{equation}
where $\mathbf{e}$ is an input embedding and $W_f$ is the parameter matrix of $f$.
% and $\Lambda(\cdot)$ is the \textit{stop gradient} operation, i.e., the gradient of $f(\mathbf{e})$ will not back propagate through $\mathbf{e}$, but only affect $W_f$.  \red{$\mathbf{e}$ \& $\Lambda$?}
% \cx{not clear what e is, because you first introduce it as a virtual concept/notation, and then fill them with the X selected next. Discuss how you construct the task first and then use e as a subset sampled from the classification triples you introduced?}
% \cx{the definition of X makes it confusing. It varies from eqn 1 to eqn 3 and 4, sometimes it is source triple, or source/target q-d pair. I suggest use X to denote (q, d) pair, $x^s$ and $x^t$ as target, $y^s$ as label, and say ANCE samples $X^s, y^s$ for $y^s=-1$. Then e enumerates $X^s$ and $X^t$. using subscript $T$ confuses with $t$, switch to sth like k or i to denote iteration.}

In order to robustly push for domain invariant representations, the domain classifier needs to provide an accurate estimation of the domain boundary.
However, as mentioned in \Cref{sec:intro}, the embedding space of DR is more scattered compared to many classification tasks, and the domain boundary estimated from a single batch can be noisy and far away from the optimal boundary.

As illustrated in \Cref{fig:model}, in order to train the domain classifier more effectively, we maintain a \textit{momentum queue} $Q$, constructed as follows.
At each iteration, we sample query--document pairs $x^t$ from the target domain, encode embeddings for $x^s$ and $x^t$, and add the \textit{detached} embeddings to $Q$:
\begin{equation}
    Q = [ \mathbf{e}_{q^s}, \mathbf{e}_{d^s}, \mathbf{e}_{q^t}, \mathbf{e}_{d^t}, \cdots ], \quad
    (q^s,d^s)=x^s, (q^t,d^t)=x^t.
\end{equation}
$Q$ contains embeddings of $x^s$ and $x^t$ pairs of the $n$ most recent batches, and $n$ is the \textit{momentum step}.
Among the chosen $x^s$, we make sure the ratio of $y^s=1$ and $y^s=0$ is $1:1$.
Here, $\mathbf{e}$ is the \textit{detached} embedding;
for example, for the query $q^s$,
\begin{equation}
    \mathbf{e}_{q^s} = \Phi(g(q^s; \theta_g)),
\end{equation}
where $\Phi$ is the \textit{stop-gradient} operator, i.e., gradients of $\mathbf{e}_{q^t}$ will not be back propagated to $\theta_g$.

At each iteration, the domain classifier is updated by minimizing the following discrimination loss:
\begin{equation}
    L_D(\mathbf{e};f) =
    \begin{cases}
        -\log f(\mathbf{e}), & \mathbf{e} \text{ from source,} \\
        -\log (1-f(\mathbf{e})), & \mathbf{e} \text{ from target,} \\
    \end{cases}
\end{equation}
\begin{equation}
    \min_{W_f} L_D(\mathbf{e}; f),
    \quad \mathbf{e} \in Q, \label{eqn:min-wf}
\end{equation}
where $L_D$ is a standard two-class classification loss to distinguish the source/target domain input embeddings.
In this way, the domain classifier is trained with signals from multiple batches, leading to faster and more robust convergence to the optimal domain boundary.
It is worth noting that since the embeddings stored in Q are detached, gradients will not be further back propagated, but only update $W_f$ as shown in \Cref{eqn:min-wf}.
In this way, efficiency of the momentum training is greatly improved since redundant forward and backward propagations through the large encoder model are saved.

% \cx{describe it from the momentum angle, that we maintain a momentum queue that keeps the samples from previous batches, and it is momentum in a way that only the final embeddings are used to update $f_D$ which is very efficient cause you can keep a big momentum queue.}

% We take inspiration from ANCE's asynchronous updating idea:\ the DR encoder's update is slow and smooth enough so that encoded embeddings from many iterations ago are still informative for the current embedding space.
% \cx{assuming batch size 1 is confusing. You can just use sth like $Q_\text{Mom}=X_{T-{NB}:T}$}


% \cx{you used different subscript for source and target in q and d, why not use $x^s$ instead of introducing y? y is often used to refer to ground truth label. The subscript sometimes refers to data point index sometimes refers to source-target, which is confusing. Use superscript to denote source-target. I prefer to use X to denote the set of data, not x. Also your x include training label which is strange.}
% \cx{People use h as BERT's output. use a different notation.}
% \cx{You never described the exact detail of h. I don't see the benefit of describing the entire model with such abstraction. It does not make this paper reads more theory instead way less clear. 
% It doesn't provide sufficient detail for people to grab what you actually do here. We used one specific setup with BERT dual-encoder, so we should directly define what our h and g are.}


% \cx{you can define what c is here. however I like to use $f_{D}$ as $c$ to pair with $L_D$.}

% \cx{you did not make it clear that the classifier do not train embeddings but only the $f_D$'s parameter, and why that will work and the benefit of it. maybe use explicitly stop gradient operation to show that it is only embeddings used as fixed input to classifier, or use explicit $argmax_{W}sum_{e \in Q} f_D(e;W)$ to make it clear.}


\subsection{Training Domain Invariant Representations with Adversarial Loss}
The encoder $g$ is adversarially updated to generate domain invariant representations that the domain classifier $f$ cannot distinguish, by minimizing an adversarial loss $L_M$.
We use the Confusion loss described in ADDA~\citep{adda}, and the adversarial loss for a query--document pair $x$ is:
% \cx{which introduce the other two losses not used in your main model here? They are ablation studies so only discuss them later when needed.}
\begin{equation}
    % l_M(y) &= -\frac{1}{2}\log h(g(y)) -\frac{1}{2}\log (1-h(g(y))), \\
    L_M(x; g, f) = -\frac{1}{2}\Big(\log f(g(q)) +\log (1-f(g(q))) +\log f(g(d)) +\log (1-f(g(d)))\Big).
\end{equation}
% \cx{The use of $X_T$ makes it unclear here again. Use sth like $x \in (q^s, d^s, q^t, d^t)$ is way better and reduces reader's effort.}
The Confusion loss reaches its minimum when the embeddings are domain invariant and impossible for the domain classifier to distinguish.
% \cx{confused is a negative word. we want domain invariance not a confused classifier. It is not the classifer being confused and don't do a good work it is our DR encoder learns true domain invariance which makes it impossible to classify.}
When pushing for domain invariance, we freeze the domain classifier and update parameters of the encoder:
\begin{equation}
    \min_{\theta_g} \sum_{x \in \{x^s, x^t\}} \lambda L_M(x; g, f) \label{eqn:loss-adversarial}
\end{equation}
% \cx{you defined Q and not use it in Eqn (8).}
We use the hyperparameter $\lambda$ to balance the learning of DR ranking in the source domain (\Cref{eqn:loss-ranking}) and the learning of domain invariance (\Cref{eqn:loss-adversarial}).

\input{fig-model}

% \cx{This inspiration is confusing. We are doing the standard momentum approach, where the embeddings in the queue are not updated. It has nothing to do with ANCE (and the gaps in momentum and ANCE's async updates are quite different. Our technique is momentum-steaming, not async update.}

% \cx{I prefer to discuss this momentum classifier as part of the discrimination loss. Describing the basic discrimination loss first and then update it with momentum (as what it is now) introduces an extra layer for readers to understand and clutter the notation (you used same $L_D$ for Eqn  (3) and Eqn (8) which is unclear anyway).
% }
% \cx{Splitting 2.3 from 2.2 also makes an impression that our contribution is only half a page worthy, which is not the case. Although ADDA is a classic method, we are the first to introduce them to ZeroDR, a new and important task (Sec 2.2) which is a novel contribution itself, though perhaps itself is quite incremental, however, we also found the unique challenge of DR for ADDA and provides a momentum solution to address it, which is novel. These two things should go together as one story, not as two subsections which look like we only make a tiny update of other's method.}


% \cx{Section 2 needs a new writing, perhaps it is the most important thing after having the 1st draft of the rest. To sumup the main problems:
% \begin{enumerate}
%     \item The story line is scattered and splitting sec 2.2 and 2.3 makes it worse. There is no motivation and definition of why/what is ZeroDR.
%     \item The description of our approach is too abstract, we should make it clear both what the high level framework and also what our exact method details are. 
%     \item The notations are wrong and need a new redesign. Several high level rules: 1) stick with common usages of symbols, e.g., X is data and Y is label, h is bert output, etc. 2) each formatting (bold, capitalization, subscript and superscript) only uses for one purpose. subscript is for data point, super for source-target, and define the momentum queue use a Set of X, Y is one solution.
%     \item I prefer to have notation definition and motivation in the paragraph and equations as separate lines, mixing equations in the paragraph is hard to read.
%     \item always have a clear outline for our main method description first and lead readers with general framework in the beginning. Letting the readers try to figure out the general picture themselves often leads to confusion.
%     \item Try keep in mind what our main contributions and main story are. Spend space and effort for parts based on their importances for this paper. 
% \end{enumerate}
% }

